Generalizing Trust: Weak-to-Strong Trustworthiness in Language Models

The rapid proliferation of generative AI, especially large language models, has led to their integration into a variety of applications. A key phenomenon known as weak-to-strong generalization - where a strong model trained on a weak model's outputs surpasses the weak model in task performance - has gained significant attention. Yet, whether critical trustworthiness properties such as robustness, fairness, and privacy can generalize similarly remains an open question. In this work, we study this question by examining if a stronger model can inherit trustworthiness properties when fine-tuned on a weaker model's outputs, a process we term weak-to-strong trustworthiness generalization. To address this, we introduce two foundational training strategies: 1) Weak Trustworthiness Finetuning (Weak TFT), which leverages trustworthiness regularization during the fine-tuning of the weak model, and 2) Weak and Weak-to-Strong Trustworthiness Finetuning (Weak+WTS TFT), which extends regularization to both weak and strong models. Our experimental evaluation on real-world datasets reveals that while some trustworthiness properties, such as fairness, adversarial, and OOD robustness, show significant improvement in transfer when both models were regularized, others like privacy do not exhibit signs of weak-to-strong trustworthiness. As the first study to explore trustworthiness generalization via weak-to-strong generalization, our work provides valuable insights into the potential and limitations of weak-to-strong generalization.

==> old_sections/section0_new.tex <==
The rapid proliferation of generative AI, especially large language models (LLMs), has spurred their deployment across diverse applications.
A key phenomenon known as weak-to-strong generalization -- where a robust model fine-tuned on a weaker model’s outputs outperforms the original model -- has sparked considerable interest. 
Yet, whether critical trustworthiness properties such as robustness, fairness, and privacy can generalize similarly remains an open question.
In this work, we study this question by examining if a stronger model can inherit trustworthiness properties when fine-tuned on a weaker model’s outputs, a process we term weak-to-strong trustworthiness generalization. 
To address this, we introduce two novel approaches: 1) Weak Trustworthiness Finetuning (Weak TFT), which leverages trustworthiness regularization during the fine-tuning of the weak model, and 2) Weak and Weak-to-Strong Trustworthiness Finetuning (Weak+WTS TFT), which extends regularization to both weak and strong models.
Our experiments on benchmark datasets reveal that while some trustworthiness properties such as fairness, adversarial, and out-of-distribution robustness show considerable improvement with regularization, others, like privacy, remain resistant to weak-to-strong transfer.
As the first work to probe trustworthiness generalization via weak-to-strong generalization, this study offers critical insights into the capabilities and limits of weak supervision.
Our findings underscore the importance of systematic trustworthiness generalization studies to develop AI systems that are not only high-performing but also reliable for real-world applications.

==> old_sections/section1_new.tex <==
Over the past few years, there has been a rapid proliferation of generative artificial intelligence (AI), particularly large language models (LLMs) like GPT-3, GPT-4, and their successors. 
These models have demonstrated remarkable capabilities across a wide range of tasks, including language comprehension \citep{radford2019language}, reasoning \citep{bubeck2023sparks} and tabular data generation \citep{borisov2022language}. 
Their emergent behaviors -- unexpected capabilities that arise as models scale -- have captured the attention of both academia and industry, leading to widespread adoption and integration into various applications \citep{wei2022emergent,schaeffer2024emergent}.

One intriguing key phenomenon observed in LLMs is known as weak-to-strong generalization \citep{burns2023weak}. 
In this context, a ``weak" model, typically smaller in terms of the number of model parameters, is used to supervise the training of a larger-sized ``weak-to-strong" model.
Remarkably, this larger model often surpasses the weak model in performance, even when trained solely on the weak model's outputs. 
Prior research has shown that when a large model is fine-tuned on the predictions of a smaller model for tasks like sentiment analysis or machine translation, the larger model not only learns the task but also generalizes better to unseen data \citep{burns2023weak}.

While performance improvements are valuable, trustworthiness has emerged as a critical aspect of AI systems, especially as LLMs are increasingly deployed in high-stakes domains like healthcare, finance, and legal services \citep{wang2023decodingtrust}.
Trustworthiness encompasses properties such as fairness (avoiding biases against certain groups), privacy (protecting sensitive information), and robustness (maintaining performance under adversarial conditions or distribution shifts). 
Ensuring these properties is essential to prevent harmful outcomes, comply with regulations, and maintain public trust in AI technologies. 
Given the importance of trustworthiness, fundamental yet unexplored questions arise:

\sidecaptionvpos{figure}{c}
\begin{SCfigure}
\centering
\includegraphics[width=.50\linewidth]{figures/teaser_wts.pdf}
\caption{\textbf{Weak-to-strong transfer strategies}.
We explore the transfer of trustworthiness properties to strong models using different weak-to-strong transfer approaches. 
\textbf{Top}: In \emph{No TFT}, both the weak and WTS models are finetuned solely for task performance.
\textbf{Middle}: In \emph{Weak TFT}, the weak model is fine-tuned for both task performance and trustworthiness, while the WTS model is finetuned only for task performance.
\textbf{Bottom}: In \emph{Weak+WTS TFT}, both models are fine-tuned for task performance and trustworthiness.}
\label{fig:teaser}
\end{SCfigure}

\newtcolorbox{question}[2][]{center,%
    colframe=green!0!black,
    colback=green!0,
    enhanced,
    attach boxed title to top left={xshift=0.5cm, yshift=-3mm},
    colbacktitle=green!0,
    coltitle=green!0!black,
    title=#2}
\begin{question}{}
\centering 
% Does the weak-to-strong generalization phenomenon extend to trustworthiness properties? \\
\emph{\textbf{Research Question}: Can a strong model inherit or potentially enhance fairness, privacy, and robustness from a weak model through fine-tuning on trustworthy weak model outputs?}
\end{question}

%Addressing this question is crucial for developing AI systems that are not only performant but also ethically aligned and reliable in critical applications.

In this work, we investigate this critical question by exploring the transfer of trustworthiness properties from weak to strong models, a process we term \emph{weak-to-strong trustworthiness generalization}. 
We specifically examine whether a strong model can inherit and enhance the trustworthiness properties of a weak model, in addition to improving task performance. 
To this end, we 
% leverage the weak-to-strong generalization framework and
introduce two novel fine-tuning strategies aimed at enhancing trustworthiness transfer.
First, we apply trustworthiness regularization during the fine-tuning of the weak model only. 
This involves modifying the loss function of the weak model to include fairness, robustness or privacy constraints.
We refer to this training strategy as \emph{Weak Trustworthiness Fine-tuning} (Weak TFT).
Second, in addition to using a trustworthiness regularized weak model, we also add trustworthiness regularization to the weak-to-strong transfer where we finetune the weak-to-strong model using a trustworthiness regularizer on the trustworthy weak labels.
We call this second strategy \emph{Weak and Weak-to-Strong Trustworthiness Fine-tuning} (Weak+WTS TFT). 
These training strategies are summarized in Figure \ref{fig:teaser}.

We conduct rigorous empirical experiments using the Pythia model suite \citep{biderman2023pythia} to evaluate these training strategies on multiple real-world datasets including Adult (fairness), OOD Style Transfer (OOD robustness), AdvGLUE++ (adversarial robustness), and Enron Emails (privacy).
Our results demonstrate that while naive fine-tuning of the strong model on the standard weak model outputs only leads to limited weak-to-strong trustworthiness, our proposed training strategies significantly enhance weak-to-strong trustworthiness.
Specifically, strong models not only retain but also consistently amplify fairness and robustness properties when both models are regularized. 
%In fairness experiments, the strong model achieved a lower demographic parity difference compared to the weak model, indicating improved fairness. Similarly, robustness assessments showed that the strong model was more resilient to adversarial perturbations and out-of-distribution shifts. 
In summary, our contributions can be summarized as follows:
\begin{itemize}[leftmargin=10mm]
% \item \textbf{Weak Trustworthiness fine-tuning (Weak TFT)}: We apply trustworthiness regularization during the fine-tuning of the weak model. This involves modifying the loss function to include fairness constraints or robustness penalties.
% \item \textbf{Weak and Weak-to-Strong Trustworthiness fine-tuning (Weak+WTS TFT)}: In addition to a regularized weak model, we add trustworthy weak-to-strong transfer to finetune the strong model using a trustworthiness regularizer on the weak labels.
\item \textbf{Novel Trustworthy Learning Paradigm:} 
This is the first work to investigate if trustworthiness properties can transfer from a weak to a strong model using weak-to-strong supervision, a process we term \emph{weak-to-strong trustworthiness generalization}.
\item \textbf{Novel Training Strategies to Elicit Weak-to-Strong Trustworthiness}: We introduce two novel training strategies, Weak TFT and Weak+WTS TFT, designed to facilitate weak-to-strong trustworthiness generalization.
\item \textbf{Weak-to-Strong Trustworthiness is Feasible}: Our experiments show that trustworthiness properties can indeed be transferred and even enhanced from weak to strong models.
\end{itemize}
Our findings provide new insights into systematically transferring and scaling trustworthiness properties from weaker to stronger models. 
They suggest a viable pathway for developing trustworthy AI systems without requiring full access to model internals or extensive human supervision.
By showing that strong models can inherit and improve trustworthiness from weaker models, we lay critical groundwork for building powerful AI systems that are ethically aligned and reliable, advancing the scalable development of trustworthy AI.
%By demonstrating that trustworthiness can be effectively inherited and even enhanced through weak-to-strong generalization, we contribute to the foundational understanding necessary for aligning powerful AI systems with ethical principles.

==> old_sections/section2_new.tex <==
This work is the first to leverage regularization techniques to study if trustworthiness properties transfer from a weak to a strong model, and one of the first to study weak to strong generalization in large language models. 
Below we discuss related works for each of these topics.

%\textbf{Weak supervision.}
%Weak supervision refers to training models with limited or noisy labeled data or with labels that may not fully capture the complexity of the tasks the model is expected to perform.
%This is different from standard supervision, where precise, high-quality labels are provided for each training example.
\textbf{Model distillation.}

\textbf{Adversarial robustness.}
Machine learning model outputs can be changed by introducing minimal perturbations to a benign input, causing the model to malfunction \citep{Szegedy2014, GoodfellowSS14, MadryMSTV18}.
Several adversarial attack algorithms have been developed that can degrade a large language model's performance on natural language processing tasks such as sentiment analysis, question answering, text classification, and entailment \citep{JinJZS20, ZangQYLZLS20, wang2020t3, li2020bertattack, garg2020bae}.
Our work differs from these existing studies and is the first to examine if adversarial robustness properties can transfer from a small model to a larger model trained on the outputs of the small model.
%\map{Include some more recent works here. Say how our work differs from these.}

\textbf{Out-of-distribution robustness.}
\ls{Doesn't define OOD robustness explicitly.}
\citet{arora2021types} classify OOD into two types: (1) ``semantic shift'', which involves unseen classes during testing, and (2) ``background shift'', which refers to changes in the domain or style of text while maintaining the underlying semantic content. 
Existing methods aiming to enhance OOD robustness can be categorized as: (1) data-driven methods, such as adding adversarial perturbations \citep{advembed, lecuyer2019certified}, EDA \citep{wei2019eda}, and FreeLB \citep{zhu2019freelb}; and (2) model and training-based methods, such as label smoothing \citep{labelsmoothing} and focal loss \citep{lin2017focal}. However, recent research has pointed out that these methods still fail to meet expectations in enhancing OOD robustness and might even cause performance degradation on original in-distribution tasks, and vanilla fine-tuning remains a strong baseline \citep{boss}. 
In this work, we adopt ``adversarial perturbation'' as a representative of robustness-enhancing methods. Differing from existing work, we are the first to study how OOD robustness can be transferred from weak models to strong ones, with or without robustness-enhancing methods.


\textbf{Fairness.} Unfair outcomes can arise in language models when they inadvertently encode biases present in the training data, leading to discriminatory practices against certain groups based on sensitive attributes like race, gender, or age \citep{bolukbasi2016man}. Recent efforts to improve fairness in LLMs include data pre-processing, post-processing, and adversarial training such as augmenting training data to balance gender representations \citep{zhao2018gender} and debiasing word embeddings \citep{huang2020reducing}. Our study sets itself apart by focusing on fine-tuning LLMs using a modified loss function explicitly designed to enhance fairness. Unlike approaches that treat fairness constraints separately or apply post-processing adjustments, we integrate fairness directly into the model's learning objective during fine-tuning. 

% This integration allows the model to internalize fairness considerations, leading to more equitable outcomes without significantly compromising performance. 

% Moreover, we conduct a systematic analysis of fairness during weak-to-strong generalization, investigating the transfer of fairness throughout different levels of weak-to-strong fine-tuning.

\textbf{Model distillation and privacy.}
\ls{First define knowledge/model distillation, condense previous studies to max 2 - 3 sentences}
Prior research has explored the use of knowledge distillation as a mechanism to mitigate privacy attacks. 
One of the most prominent examples is the PATE framework \citep{papernot2016semi}, where knowledge distillation is employed to reduce an ensemble of teacher models into a single model with provable privacy guarantees \citep{dwork2006calibrating}.
Other works have built on this idea, such as \citet{zheng2021resisting} and \citet{tang2022mitigating} who construct privacy-preserving model ensembles and then use distillation to consolidate these models. 
In these approaches, knowledge distillation is often one component of a larger privacy-preserving model, which helps to build models with privacy guarantees.
Some research suggests that distillation alone can serve as an effective privacy defense \citep{shejwalkar2021membership}. Building on this, \citet{mazzone2022repeated} investigate the use of repeated distillation to protect against membership inference attacks. However, \citet{jagielski2024students} demonstrate through privacy attacks that distilled models without privacy guarantees can still leak sensitive information.
In contrast to prior work, our research focuses on the privacy implications of weak-to-strong training, where a large model is trained on the outputs of a smaller model. 
This approach is the inverse of traditional model distillation, where smaller models are typically trained using the outputs of larger models.
Relatively little is known about the privacy risks and benefits when this process is reversed, making our investigation an important contribution to the field.


==> old_sections/section3_new.tex <==
We now present our methodology for investigating the generalization of trustworthiness properties from weak to strong models.
Our approach systematically explores whether and how fairness, privacy, and robustness can be effectively inherited and enhanced by stronger models. 
The broader issue we address is: Under what conditions can a weaker model, despite its limitations, most effectively transfer properties such as fairness, privacy, and robustness to a more powerful model?
We begin by outlining the weak-to-strong training process, followed by techniques for eliciting specific trustworthiness properties in language models.
Finally, we introduce a novel three-stage approach that allows us to examine weak-to-strong trustworthiness under different fine-tuning strategies.

% A key challenge in superalignment is the need for humans to supervise models that are far more intelligent than we are \citep{burns2023weak}. 
% In the context of trustworthy AI, this raises the question of how to guide these highly capable models toward ethical and robust behavior when the supervision comes from weaker, less capable models.
% In this work, we explore this question by conducting a series of experiments where a weak model, using only its outputs, acts as a mentor for a stronger model. 
% The goal is to examine whether trustworthiness properties can be transferred from a weak model to a strong one, and under what conditions such transfer is most effective.

\subsection{Preliminaries}

Here we present the key training strategies that underlie our work. 
First, we discuss how we adapt the weak-to-strong generalization framework introduced by \citet{burns2023weak}.
Following this, we examine widely-used regularization strategies for machine learning models aimed at enhancing trustworthiness properties such as robustness, fairness, and privacy.

\textbf{Notation.} We consider training datasets of the form $\{(x_i,y_i)\}_{i=1}^N$ where $y_i \in \mathcal{Y}$ is the ground-truth label and $a_i \in \{0,1\}$ represents a protected attribute (e.g., race or gender) that may be included in the features $x_i$.
We denote a classifier $f_\theta : \mathcal{X} \to \mathcal{Y}$ parametrized by $\theta \in \mathbb{R}^d$, mapping inputs $x \in \mathcal{X}$, to labels $\mathcal{Y}$. 
We define the outputs of a smaller, already trained, fixed classifier 
$f_w(x)$ as \emph{weak labels}, where $w \in \mathbb{R}^k$ denotes a lower-capacity parameterization than $\theta$ where $k \ll d$.   
Additionally, let $\ell: \mathbb{R} \times \mathbb{R} \to \mathbb{R}$ represent an appropriate loss function such as cross-entropy loss.

% To explore whether trustworthiness properties can be transferred from a weak model to a stronger teacher model, 
% We focus on widely-used fine-tuning techniques aimed at enhancing model trustworthiness.
% Below, we outline the respective objective functions employed to encourage trustworthy behavior of the finetuned model.

\textbf{Weak-to-Strong Training.}
Knowledge transfer from a large pre-trained model occurs by fine-tuning it on the labels produced by a smaller model. This process incorporates an additional auxiliary confidence loss, weighted by $\alpha \in [0,1]$ that adjusts the confidence in the strong model's predictions relative to the weak labels. 
This auxiliary loss encourages the strong model to make confident predictions, even when they diverge from the weak labels, potentially enhancing generalization.
The loss function adapted to our weak-to-strong trustworthiness setting is defined as a linear combination of the losses from the trustworthy weak and strong models
\begin{equation}
\ell_{\text{WTS-AUX}}(x, f_\theta; \alpha, \lambda, f_w) = (1 - \alpha) \cdot \ell\big(f_\theta(x), f_w(x;  \lambda)\big) + \alpha \cdot \ell\big(f_\theta(x; \lambda), \hat{f}_{t, \theta}(x)\big),
\label{eq:objective_trustworthy_wts}
\end{equation}
where $f_w(x; \lambda)$ is the fixed trustworthy weak model previously trained with trustworthiness property regularization strength $\lambda$ and $f_\theta(x)$ denotes the strong model.
Further, $\hat{f}_{t, \theta}(x)$ represents the hardened strong model predictions according to threshold $t$ that is set proportional to the class weights for each dataset. 
When $\lambda=0$, we are in the standard weak-to-strong setting previously studied by \citet{burns2023weak}.
When $\alpha=0$, we refer to the loss as $\ell_{\text{Naive}}$ since we train on the outputs of the weak model only.
In the following, we describe how we obtain the weak trustworthy models $f_w(\cdot; \lambda)$ through various regularization techniques aimed at improving trustworthiness. 
%For each property, we select a value for $\alpha_{\max}$ that controls the $\alpha$ in WTS-Aux-Loss, as $\alpha$ linearly increases from 0 to $\alpha_{\max}$ over the first 20\% of training datapoints. $f_w(x)$ and $f(x)$ denote the weak and strong label predictive distributions, respectively. $\hat{f}_t(x)$ denotes the hardened strong model predictions according to threshold $t$ that is set proportional to the class weights for each dataset. The parameter $\alpha_{\max}$ is selected separately for each trustworthiness property (Appendix A, Figure \ref{appx:trade-off-adv}).

%\textbf{Strong Ceiling}: The large pretrained model is finetuned on ground truth labels. This establishes an upper bound on performance, representing what the strong model can achieve with perfect supervision.

% \subsection{Eliciting Trustworthiness Properties in Large Language Models}

% \map{Initial pass complete.} 

\textbf{Fairness.} 
% Given a training dataset $\{(x_i,y_i)\}_{i=1}^N$ where $y_i \in \{0,1\}$ is the label, $a_i \in \{0,1\}$ represents a protected attribute included in the features $x_i$, 
Here we discuss how we can enhance fairness through regularization using a widely-used fairness notion known as Demographic Parity which requires:
\begin{align}
\mathbb{P}(f_\theta(x) = 1 | a = 1) = \mathbb{P}(f_\theta(x) = 1 | a = 0).
\label{eq:demographic_parity}
\end{align}
To incorporate this fairness constraint in the fine-tuning process of the weak models, we employ an objective function adapted from \citet{zafar2017fairness}, 
%to align with our weak-to-strong training setting,
\begin{align}
\min_w \mathcal{L}_{\text{Fair}}(w; \lambda_{\text{Fair}}) = \min_w \frac{1}{N} \sum_{i=1}^N \ell(f_w(x_i), y_i) + \lambda_{\text{Fair}} \cdot  (a_i - \bar{a}) \cdot f_w(x_i),
\label{eq:fairness_regularizer}
\end{align}
where $\bar{a} = \frac{1}{N} \sum_{i=1}^N a_i$ is the base rate of the protected attribute. 
The first term in \eqref{eq:fairness_regularizer} encourages to make correct predictions while the second term acts as a fairness regularizer.
Specifically, this term minimizes the covariance between the protected attribute $a_i$ and the model outputs $f_w(x_i)$, encouraging the model to satisfy demographic parity by becoming independent of the protected attribute $a$.
The hyperparameter $\lambda_{\text{Fair}}$ controls the tradeoff between prediction accuracy and fairness where a higher value of $\lambda_{\text{Fair}}$ encourages more emphasis on achieving fairer outcomes. 

\textbf{Out-of-distribution robustness.} 
We use embedding perturbations as the method to enhance out-of-distribution robustness, following approaches from \citet{advembed, lecuyer2019certified, zhu2019freelb}.
Specifically, we add i.i.d.\ Gaussian noise to the word embeddings \citep{bowman2015generating, li2019certified}.
Define \(e(x) \in \mathbb{R}^{d} \) as the word embedding of input \( x \), where \( d \) is the embedding dimension.
We add Gaussian noise \(z \sim \mathcal{N}(0, \lambda_{\text{OOD}} \cdot \text{I}_d) \) drawn from a distribution with mean $0$ and covariance matrix \( \lambda_{\text{OOD}} \cdot \text{I}_d\) to the word embedding which yields a noisy embedding: \(\tilde{e}(x; \lambda_{\text{OOD}}) = e(x) + z \).
This noisy embedding is then used to finetune the model.
Here, let \( f_w(x; \lambda_{\text{OOD}}) = g_{w}(\tilde{e}(x; \lambda_{\text{OOD}})) \) be the output of the language model parametrized by $w$. 
The objective during fine-tuning is to minimize the following loss:
\begin{align} 
\min_w \mathcal{L}_{\text{OOD}}(w; \lambda_{\text{OOD}}) = \min_{w} \frac{1}{N} \sum_{i=1}^N 
\ell\big(f_w(x_i; \lambda_{\text{OOD}}), y_i\big),
\end{align}
where $\lambda_{\text{OOD}}$ controls the strength of the OOD regularizer. 
As $\lambda_{\text{OOD}} \to 0$ the model is trained without any regularization, reverting to the vanilla model. 


\textbf{Adversarial Robustness.}
% \ak{Machine learning models, such as deep neural networks, are known to malfunction under small, adversarial changes in their inputs \citep{Szegedy2014, GoodfellowSS14, MadryMSTV18}.
% Such adversarial inputs are generated using optimization procedures that seek to change the output of a model by introducing minimal perturbations to a benign input.
% Large language models (LLMs), being deep neural networks, are not exempt from this vulnerability. Several adversarial attack algorithms have been developed that can degrade an LLM's performance on natural language processing tasks such as sentiment analysis, question answering, text classification, and entailment \citep{JinJZS20, ZangQYLZLS20, wang2020t3, li2020bertattack, garg2020bae}.
% }
In adversarial training, adversarially perturbed samples are introduced during the training process, enabling the model to learn to become invariant to small input perturbations and thereby become more robust to adversarial attacks.
In this setting, the training dataset consists of triplets $(x, x', y)$, where $x$ is a clean input sample, $x'$ is an adversarially manipulated version of $x$ and $y$ is the ground truth label of $x$.
%We denote the $i^{th}$ training sample as $(x_i, x'_i, y_i)$.
%As before, let $f_\theta$ represent the model and $\ell$ be a loss function (e.g., cross-entropy loss) that measures the model's prediction accuracy. 
The training objective combines the losses from both clean and adversarial samples:
\begin{align}
\min_w \mathcal{L}_{\text{Adv}}(w; \lambda_{\text{Adv}}) = \min_w \; \frac{1}{N} \sum_{i=1}^N(1-\lambda_{\text{Adv}}) \cdot \ell(f_w(x_i), y_i) + \lambda_{\text{Adv}} \cdot \ell(f_w(x_i'), y_i),
\end{align}
where $\lambda_{\text{Adv}}$ controls the tradeoff between clean and adversarial losses. 
A higher $\lambda_{\text{Adv}}$ places greater emphasis on robustness to adversarial perturbations.

\textbf{Privacy.}
In $(\lambda_P,\delta)$-differential privacy, the goal is to ensure that the output of an algorithm $\mathcal{A}$ is nearly indistinguishable whether or not any single data point is included in the dataset. 
Specifically, for any two datasets $D_1$ and $D_2$ that differ by only one element, the algorithm $\mathcal{A}$ satisfies $(\lambda_P,\delta)$-differential privacy if:
\begin{align}
\mathbb{P}(\mathcal{A}(D_1) \in S) \leq \exp(\lambda_P) \cdot \mathbb{P}(\mathcal{A}(D_2) \in S) + \delta,
\end{align}
for any possible output set $S$. 
Here, $\lambda_P$ controls the privacy loss, with smaller values indicating stronger privacy guarantees, while $\delta$ allows for a small probability of the privacy guarantee being violated.
To operationalize $(\lambda_{P}, \delta)$-differential privacy, we use the most popular privacy algorithm called DP-SGD as in the work by \citet{abadi2016deep}, which is a variant of classical SGD that comes with privacy guarantees.
In summary, the algorithm consists of three fundamental steps: 
\emph{gradient clipping} with clipping constant $C$, i.e., $\gamma = g(x_i, y_i) \cdot\max(1, C/\lVert g(x_i, y_i)\rVert)$ where $g(x_i, y_i) = \nabla_\theta \mathcal{L}(x_i, y_i)$ is the gradient of the loss function $\ell$ with respect to the model parameters,
\emph{aggregation} (i.e., $m = \frac{1}{n}\sum_{i=1}^n \gamma_i$) and
\emph{adding Gaussian noise} (i.e., $\tilde{m} = m + Y$ where $Y \sim \mathcal{N}(0, \tau^2 \text{I})$ with variance parameter $\tau^2$).
By carefully tuning the noise level $\tau^2$, we ensure that the model satisfies the privacy guarantees specified by the parameters $\lambda_{P}$ and $\delta$.
Everything else equal, for a specified $\delta$, a higher noise level implies a lower $\lambda_{P}$ and thus better privacy guarantees.

\subsection{Eliciting Weak-to-Strong Trust in Large Language Models}
\label{sec:training_strategies}
In this Section, we present the methodology to study weak-to-strong trustworthiness.
We break the analysis into three training strategies, each building on the last by varying the regularization applied to the weak and weak-to-strong models, respectively.

% \ak{Suggestion for phase names:
% \begin{itemize}
%     \item Phase 1: No Trustworthiness Fine-Tuning (No TFT)
%     \item Phase 2: Weak (model) TFT
%     \item Phase 3: Weak + Weak-to-Strong TFT (Weak + WTS TFT)
% \end{itemize}
% }

\textbf{No trustworthiness fine-tuning (No TFT).}
This training strategy establishes baseline performance by training the weak, strong, and weak-to-strong models without applying any trustworthiness regularization, following the approach outlined in \citet{burns2023weak}:
\begin{enumerate}[label=\(\bullet\), leftmargin=4mm, nosep]
\itemsep0.10cm
\item \textbf{Weak model:} 
We use small, pretrained LLMs as weak supervisors, referred to as weak models.
These weak models are finetuned on ground truth labels to generate predictions. 
Using the resulting finetuned weak models $f_w(\cdot, \lambda)$ where $\lambda=0$, we create weak labels by having the weak models make predictions on a held-out validation set.
\item \textbf{Weak-to-strong transfer:}  
To train weak-to-strong models, we fine-tune a strong model using the weak labels generated by the weak model using \eqref{eq:objective_trustworthy_wts}. 
This model is referred to as the strong student, and its resulting performance is called the weak-to-strong performance.
% \item \textbf{Strong ceiling:} 
% For comparison, we also fine-tune a strong model using the actual ground truth labels. 
% This is referred to as the strong ceiling model, and its performance represents the upper bound of what the strong model can achieve when fully utilizing its capabilities on the task.
\end{enumerate}

\textbf{Weak trustworthiness fine-tuning (Weak TFT).}
This training strategy explores whether a trustworthiness regularized weak model can influence the trustworthiness property of a vanilla strong model trained solely on the output of the trustworthy weak model:
\begin{enumerate}[label=\(\bullet\), leftmargin=4mm, nosep]
\itemsep0.10cm
\item \textbf{Trustworthy weak model:}
We use small, pre-trained LLMs as weak supervisors, but unlike in Phase 1, these weak models are fine-tuned on ground truth labels using a trustworthiness regularizer. 
This regularizer enforces specific trustworthiness properties, such as fairness, privacy, or robustness, during fine-tuning. These models are referred to as trustworthy weak models.
Using these trustworthy weak models $f_w(\cdot, \lambda)$ where $\lambda>0$, we generate weak labels by making predictions on a held-out validation set.
\item \textbf{Weak-to-strong transfer:} 
To assess whether trustworthiness properties can be transferred from a weak to a strong model, we fine-tune a vanilla strong model using the weak labels generated by the weak model using \eqref{eq:objective_trustworthy_wts}. 
% This model is called the implicit trustworthy strong student, and its performance, referred to as implicit trustworthy weak-to-strong performance, reflects how well the strong model incorporates trustworthiness properties from the weak model.

% \item \textbf{Trustworthy strong ceiling:} 
% For comparison, we fine-tune a trustworthy strong model using the ground truth labels, applying the same trustworthiness regularizer used for the weak model. 
% This model is called the trustworthy strong ceiling model, and its performance represents the maximum possible capability of the strong model when trained with both ground truth labels and trustworthiness properties.
\end{enumerate}

\textbf{Weak and weak-to-strong trustworthiness fine-tuning (Weak+WTS TFT).}
The last training strategy investigates whether adding trustworthiness regularization to both the weak and weak-to-strong models can further enhance trust transfer (and performance).
\begin{enumerate}[label=\(\bullet\), leftmargin=4mm, nosep]
\itemsep0.10cm
\item \textbf{Trustworthy weak model:} The trustworthy weak model is the same as in the Weak TFT training strategy, where the weak model is fine-tuned on ground truth labels using a trustworthiness regularizer to enforce properties like fairness, privacy, or robustness.
\item \textbf{Trustworthy weak-to-strong transfer:}
In this step, we directly assess how well trustworthiness properties can be transferred from the weak model to the strong model. Unlike for the previous training strategy, where the strong model was fine-tuned without any regularization, here we finetune the strong model using a trustworthiness regularizer on the weak labels generated by the trustworthy weak model. We provide details on this training objective in Appendix \ref{app:objective_third_stage}.
 % This model is referred to as the doubly trustworthy strong student, and its performance, called doubly trustworthy weak-to-strong performance, measures how effectively the strong model incorporates trustworthiness properties when both models are regularized.
% \item \textbf{Trustworthy strong ceiling:} The trustworthy strong ceiling model is the same as in Phase 2, where the strong model is fine-tuned on ground truth labels with trustworthiness regularization, representing the upper limit of performance with respect to trustworthiness.
\end{enumerate}


==> old_sections/section4_new.tex <==
\newtcolorbox{takeaway}[2][]{center,%
    colframe=green!0!black,
    colback=green!0,
    enhanced,
    attach boxed title to top left={xshift=0.5cm, yshift=-3mm},
    colbacktitle=green!0,
    coltitle=green!0!black,
    title=#2}

% We now present our empirical analysis.
In Section \ref{sec:experiments_main}, we empirically evaluate the effectiveness of generalizing trustworthiness properties from a weak to a strong model using the three weak-to-strong training strategies introduced in the previous section.
Then, in Section \ref{sec:experiments_sensitivity}, we perform a thorough sensitivity analysis, varying the trustworthiness regularization strength, model size, and key hyperparameters specific to weak-to-strong transfer training. 
We begin by describing the real-world datasets used in our experiments, followed by an overview of the LLMs and relevant baselines used for comparison.

\textbf{Datasets.} 
We evaluate the transfer of trustworthiness properties from small models to large models using four datasets, previously explored by \citet{wang2023decodingtrust}, including the Enron Email dataset \citep{klimt2004enron}, the Adult dataset \citep{ding2021retiring}, the OOD Style Transfer dataset \citep{wang2023decodingtrust}, and the AdvGLUE++ dataset \citep{wang2023decodingtrust}. 
For all datasets, we show average results over multiple runs and usually report $\pm 1$ standard deviation across runs. 
\begin{enumerate}[label=\(\bullet\), leftmargin=3mm, nosep]
\itemsep0.10cm
\item \textbf{Adult}: This dataset is derived from the 1994 U.S. Census database and contains 48,842 instances with 14 attributes.
The task is to classify whether an individual’s income exceeds \$50,000 (USD) per year. We use the reconstructed Adult dataset provided by \citet{ding2021retiring} and selected the ``sex'' feature as the protected attribute to evaluate fairness-related properties.
\item \textbf{OOD Style Transfer}: This dataset is based on the SST-2 sentiment classification dataset but incorporates a variety of text and style transformations. 
The transformations (e.g., shifts in language style, vocabulary, syntax, and tone) are applied at both the word and sentence level while preserving the original meaning. 
For instance, some transformations involve substituting words with Shakespearean equivalents.
The task is to correctly classify the sentiment of inputs. %despite these style transformations.
\item \textbf{AdvGLUE++}: This dataset contains clean and adversarial input 
samples for six NLP tasks: Sentiment analysis (SST-2), duplicate question detection (QQP), multi-genre natural language inference (MNLI, MNLI-mm), recognizing textual entailment (RTE), and question answering (QNLI).
It contains around 2K to 15K samples for each of the six tasks.
We randomly sample up to 10K samples for each task and aggregate the performance of the model by averaging over these six tasks.
\item \textbf{Enron Emails}: This dataset contains over 600,000 emails generated by employees of the Enron Corporation.
This dataset includes sensitive personal information, such as email addresses, phone numbers, credit card numbers, and Social Security Numbers, which could be memorized and extracted by language models. 
For fine-tuning, we randomly subsampled 10,000 data points.
\end{enumerate}

\textbf{Large Language Models.} We conduct our experiments using the Pythia model suite \citep{biderman2023pythia}, which includes models of varying scales (14M, 70M, 410M, 1B). 
This allows us to systematically explore how model size impacts the effectiveness of weak-to-strong trustworthiness generalization. 
For each model, we finetune on classification tasks by adding a classification head on top of the second-to-last layer. 
The models are trained using the standard cross-entropy loss. %, with an initial learning rate of $5 \cdot 10^{-5}$.

\textbf{Metrics.} We evaluate the trustworthiness properties across small, large and weak-to-strong models using the following metrics:
\begin{enumerate}[label=\(\bullet\), leftmargin=3mm, nosep]
\itemsep0.10cm
\item \textbf{Fairness}: We evaluate the finetuned LLMs  using the Demographic Parity Difference (DPD) defined as
$\text{DPD} = \mathbb{P}(f_\theta(x) = 1 | a = 1) = \mathbb{P}(f_\theta(x) = 1 | a = 0)$.
A smaller DPD indicates better fairness, as it reflects minimal disparity in predictions between the two protected groups.
\item \textbf{Robustness}: We measure both OOD accuracy and adversarial accuracy, abbreviated as Robust Accuracy (RA), by evaluating the model's performance on OOD and adversarially perturbed test data.
Specifically, we compute the $\text{RA} = \frac{1}{n_{\text{test}}} \sum_{i=1}^{n_{\text{test}}} \mathbb{I}[f_\theta(x_i') = y_i]$, where $x'$ represents either an OOD sample or an adversarially perturbed input, and  $\mathbb{I}$ is the indicator function that equals 1 if the prediction is correct.
\item \textbf{Privacy}: We evaluate the models using targeted data extraction attacks \citep{carlini2021extracting}.
In this attack, given a prefix sequence and a generated response of $k$ tokens, we compute the extraction rate by determining what fraction of the $k$-token continuation (suffix) matches the ground truth continuation of the sample. 
A higher extraction rate indicates a greater risk of private information being memorized and extracted by the model.
\end{enumerate}

\textbf{Baselines.}
For comparison, we establish reference points for both trustworthiness and task performance.
To provide a benchmark, we fine-tune a strong model using ground truth labels with varying levels of trustworthiness regularization. 
We then select the model that achieves the best trade-off between task performance and trustworthiness. 
We provide an illustrative example of this selection procedure in Figure \ref{fig:tradeoff}.
This model, referred to as the \emph{strong ceiling}, represents the empirical upper bound of the strong model’s capabilities for both task performance and trustworthiness.

%\subsection{Experimental Setup}
%datasets
%models
%parameter settings
%metrics
%methods (strong ceiling, weak model, weak to strong transfer) 
%use macros for strong ceiling, weak model, wts transfer etc. 

\subsection{Evaluating Trustworthiness of the Weak to Strong Model}
\label{sec:experiments_main}

%\map{First pass complete. Potentially talk about task performance.}
We present our results for all four trustworthiness properties across the three phases in Table \ref{tbl:wts_table} and Figure \ref{fig:experiment_main}. We define weak-to-strong trustworthiness as the trend of the WTS-Naive and WTS-Aux-Loss models being more trustworthy than the weak model, and the strong ceiling being more trustworthy than the WTS-Naive and WTS-Aux-Loss models.

For each property, we used Pythia 14M as the weak model and Pythia 410M as the strong model.

\begin{figure}[tb]
\centering
\begin{subfigure}{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/fairness_main_results.png}
\caption{Fairness}
\label{fig:main_fairness}
\end{subfigure}~
\begin{subfigure}{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/ood-main.pdf}
\caption{OOD Robustness}
\label{fig:main_ood_rob}
\end{subfigure}~
\begin{subfigure}{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/pythia-14m-410m-ep6.png}
\caption{Adv.\ Robustness}
\label{fig:main_adv_rob}
\end{subfigure}~
\begin{subfigure}{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/privacy_main_plot_14-410.png}
\caption{Privacy}
\label{fig:main_privacy}
\end{subfigure}

\caption{\textbf{Weak-to-strong trustworthiness for Pythia 14M/410M models}. {Trustworthiness properties and task performance for our four properties: Fairness, OOD Robustness, Adversarial Robustness, and Privacy. Note that lower values are better for the top plot in Figure \ref{fig:main_fairness} as the y-axis is Unfairness (DPD). Similarly, lower values are better for the top plot in Figure \ref{fig:main_privacy} as the the y-axis is Extraction Rate.} Results for WTS-Aux-Loss for privacy are omitted since it was the only task involving free data generation, making the auxiliary loss function inapplicable.}
\label{fig:experiment_main}
\end{figure}


\begin{table}[tb]
\centering
\begin{tabular}{ccccc}
\toprule
& \textbf{Fairness}  & \textbf{\begin{tabular}[c]{@{}c@{}}OOD \\ Robustness\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Adv.\ \\ Robustness\end{tabular}} & \textbf{Privacy} \\ 
\midrule
\textbf{No TFT} & $\times$ & $\checkmark$ & $\checkmark$ & $\times $ \\ \midrule
\textbf{Weak TFT} & $\times$ &  $\checkmark$  & $\times$ & $\times$  \\ \midrule
\textbf{Weak+WTS TFT} &  $\checkmark$ &  $\checkmark$ &  $\checkmark$ & $\times$ \\ \bottomrule
\end{tabular}
\centering
\caption{\textbf{Presence of weak-to-strong trustworthiness across trustworthiness properties for different training strategies.} For the No TFT and Weak TFT training strategies, we observe inconsistent weak-to-strong trustworthiness. In Weak+WTS TFT stage, we observe consistent significant trustworthiness WTS across fairness, OOD robustness, and adversarial robustness. Privacy does not display trustworthiness WTS in any stage.}
\label{tbl:wts_table}
\end{table}

\textbf{No TFT.}
% \ls{takeaway first sentence? or italics?}
For the baseline No TFT training strategy, where models are trained without any trustworthiness regularization, we expected no clear weak-to-strong trustworthiness trends, as no regularization is in place to explicitly enforce trustworthiness properties.
Surprisingly, for both OOD and adversarial robustness evaluation we observe that the models demonstrate a weak-to-strong trustworthiness trend. 
Despite the absence of regularization, the stronger models exhibited improved robustness compared to the weaker models, suggesting that some trustworthiness properties may naturally transfer even without explicit constraints.
For fairness, we do not observe a weak-to-strong trustworthiness trend. 
The level of unfairness remains constant, regardless of whether we examine the weak model or the weak-to-strong model.  
Finally, privacy presents a unique situation. 
Note that the strong ceiling does not achieve better privacy than the weak model.
One reason for this is that we measure the privacy property with respect to the underlying training dataset. 
Larger models, all else being equal, tend to memorize more information, leading to a greater risk of private information leakage \citep{leemann2024gaussian} and as a result larger models are more susceptible to leak private data than small models.
As a result, we observe that privacy, as measured by the extraction rate, degrades when transferring knowledge from the smaller model to the larger model, primarily because privacy violations for WTS-Naive are measured for the larger model, which is more capable of memorizing its training data, rather than the smaller one.

\begin{takeaway}{}
\centering 
\emph{\textbf{Takeaway 1}: Without trustworthiness fine-tuning, we observe inconsistent weak-to-strong trustworthiness trends.}
\end{takeaway}

%On the task performance side, only the models for OOD robustness and privacy displayed weak-to-strong trends. Their WTS-Naive model outperforms their weak model in percentage of accurate predictions, with OOD robustness' WTS-Aux-Loss models achieving similar performance as the WTS-Naive models. There is no task performance weak-to-strong for fairness or adversarial robustness as their weak models slightly outperforms their WTS-Naive and WTS-Aux-Loss models. \ls{mention there is little gap between weak and strong performance in Phase 1?} 

\textbf{Weak TFT.}
In the Weak TFT phase, regularization is applied to the weak models, which, as expected, improves their trustworthiness in terms of fairness, OOD robustness, and adversarial robustness compared to the No TFT phase. 
This improvement aligns with our expectations, as the weak models are now being explicitly regularized to enhance their trustworthiness.
\emph{The only weak-to-strong trustworthiness trend observed in the Weak TFT phase pertains to OOD robustness.} 
In this case, the improvement is substantial, increasing robust accuracy from 72\% for weak model to 75\% for WTS-Naive and WTS-Aux-Loss, representing a gain of 3 percentage points.
For all other cases, we do not observe weak-to-strong trends.
For fairness, the weak, WTS-Naive, and WTS-Aux-Loss models are more fair in Weak TFT compared to in No TFT, but still do not display trustworthiness WTS.
For adversarial robustness, the weak model improves significantly to 78\% robustness (from 71\% in No TFT). While the WTS-Naive and WTS-Aux-Loss improve relative to their robustness in No TFT, they are not able to surpass the weak model in Weak TFT; weak-to-strong trustworthiness no longer holds.
For privacy, while we do not observe a weak-to-strong trustworthiness trend, the gap in extraction rates between the WTS-Naive model and the weak model widens. 
This widening occurs because the smaller model benefits from privacy regularization, which limits the leakage of information about the training data. 
In contrast, the WTS-Naive model is trained without any regularization on a second, disjoint dataset, meaning the privacy guarantees from the first model's training phase do not apply. 
As a result, without explicit regularization during WTS training, the extraction rate for the explicitly regularized weak model decreases much more rapidly, dropping from 18\% to 14\%. In contrast, the implicitly regularized WTS-Naive model, trained on the outputs of the weak model, experiences a much smaller decline in extraction rate, from 45\% to 44\%.

\begin{takeaway}{}
\centering 
\emph{\textbf{Takeaway 2}: Weak trustworthiness fine-tuning improves the trustworthiness properties of weak and WTS models, but does not lead to additional weak-to-strong trustworthiness trends.}
\end{takeaway}

%Weak TFT does not result in change in extraction rate or task performance for privacy. 

%we notice that the weak model trustworthiness improves relative to the No TFT phase. However, the only weak-to-strong trustworthiness trend in the Weak TFT phase is for OOD robustness.

\textbf{Weak+WTS TFT.} 
The Weak+WTS TFT phase introduces an additional layer of trustworthiness to the weak-to-strong transfer process, as the training of the WTS model itself is now regularized on top of the existing regularization applied to the weak model in the Weak TFT phase.
\emph{With both weak and weak-to-strong models fine-tuned using a trustworthiness regularizer, we observe consistent weak-to-strong trends for all trustworthiness properties, except for privacy.}
For fairness, OOD robustness, and adversarial robustness, we observe a statistically significant improvement of each property from weak models to WTS-Naive models. In addition, for fairness and adversarial robustness, there is an enhanced transfer from weak to WTS-Aux-Loss (where WTS-Aux-Loss is more trustworthy than WTS-Naive). 
For privacy, the extraction rate of the WTS-Naive model decreases by approximately 20 percentage points, dropping from 45\% to 26\%. 
This indicates an improvement in privacy compared to the WTS-Naive models from the No TFT and Weak TFT phases, attributed to the explicit regularization applied during WTS-Naive training.
However, despite this regularization, the WTS-Naive model remains less private than the weak model, which has an extraction rate of 14\%.

\begin{takeaway}{}
\centering 
\emph{\textbf{Takeaway 3}: Consistent weak-to-strong trustworthiness trends emerge for fairness, OOD and adversarial robustness under Weak+WTS trustworthiness fine-tuning.}
\end{takeaway}

\textbf{Tradeoff Between Trustworthiness and Task Performance.} For fairness and adversarial robustness, improvements in trustworthiness came with a slight decline in task performance. However, the decrease in accuracy does not exceed 1.5\% across all phases for the two properties while the improvements in trustworthiness were up to 3 percentage points (equivalent to 60\% decrease in unfairness). This demonstrates that significant enhancements in trustworthiness can be achieved with minimal sacrifice to task performance.

% \citep{leemann2024gaussian}.
% The strong ceiling does not achieve better privacy than the weak model. While WTS-Naive model outperforms the weak model in task performance, we do not observe a weak-to-strong trend in privacy as the WTS-Naive model is less private than both the weak model and strong ceiling.
% \ls{@Martin, explain that Privacy has no WTS-Auxiliary, also elaborate on intuition for why WTS is not present even if you fine-tune for privacy, also touch upon how task performance is defined differently for weak and WTS models (trained dataset vs ground truth)}

% We observe a tradeoff between trustworthiness and task performance (accuracy on initial task) for all properties but OOD robustness. For fairness and adversarial robustness, trustworthiness for weak model improves from the No TFT phase to the Weak TFT and Weak+WTS TFT phases, resulting in a decline in weak model task performance. There is a similar tradeoff of a smaller scale for applying WTS-Naive and WTS-Auxiliary for fairness and adversarial robustness in Weak+WTS TFT phase: task performance declines by 1\% - 1.5\% but trustworthiness improves 2\% - 4\%. No tradeoff is present in OOD robustness as weak-to-strong methods significantly improve both robustness and task performance. 

\subsection{Sensitivity Analysis}
\label{sec:experiments_sensitivity}

\begin{figure}[tb]
\centering
\begin{subfigure}{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/fairness_lambda_phase3.png}
\caption{Fairness}
\label{fig:fairness_lambda_phase3}
\end{subfigure}~
\begin{subfigure}{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/ood-lambda-phase3.pdf}
\caption{OOD Robustness}
\label{fig:ood_lambda_phase3}
\end{subfigure}~
\begin{subfigure}{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/phase3_sensitivity_plots.png}
\caption{Adv.\ Robustness}
\label{fig:adv_rob_lambda_phase3}
\end{subfigure}~
\begin{subfigure}{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/privacy_sensitivity_phase3.png}
\caption{Privacy}
\label{fig:privacy_lambda_phase3}
\end{subfigure}
\caption{\textbf{Varying Lambda for Weak+WTS TFT}. Results for WTS-Aux-Loss for  privacy are omitted since it was the only task involving free data generation, making the auxiliary loss function inapplicable.}
\label{fig:lambda_phase3}
\end{figure}

In this section, we conduct a comprehensive sensitivity analysis to explore how various parameter values influence the transfer of trustworthiness properties from weak to strong models. Specifically, we examine the impact of different model sizes and the regularization strength ($\lambda_{\text{Fair}}, \lambda_{\text{Adv}}, \lambda_{\text{OOD}}, \lambda_P$) in the trustworthiness loss functions. We continue the sensitivity analysis for the auxiliary loss weighting parameter ($\alpha$) used during weak-to-strong transfer in Appendix \ref{sec:appendix_a}. This analysis aims to validate the robustness of our findings from the previous section and to understand the conditions under which weak-to-strong trustworthiness transfer is most effective.

\textbf{Sensitivity to Model Size.}
To assess the effect of model capacity on trustworthiness transfer, we experimented with different combinations of weak and strong model sizes. We analyzed experiments for four weak/strong configurations: Pythia 14M/410M, Pythia 14M/1B, Pythia 70M/410M, Pythia 70M/1B.
Our analysis reveals that the weak-to-strong trends observed in the previous section generally hold across these model sizes for most trustworthiness properties. Specifically, for fairness and OOD robustness, the strong models continued to inherit and, in some cases, enhance the trustworthiness attributes from the weak models across all configurations (Figure \ref{fig:fairness_model_size}, Figure \ref{fig:ood_robustness_model_size}).

\ls{multiple claims made here, separate?}
However, we observed a disruption of the weak-to-strong trend for adversarial robustness when using 70M as the weak model. The weak-to-strong trend in adversarial robustness was disrupted in the Weak+WTS TFT phase in the 70M/410M and 70M/1B configurations; the strong models did not exhibit the expected improvement in adversarial robustness over the weak models (Figure \ref{fig:adversarial_robusness_model_size}). This contrasts with the results from using a 14M weak model, where the strong models did show enhanced adversarial robustness. This disruption suggests that as the weak model becomes more capable, the transfer of adversarial robustness to even stronger models may not follow the same patterns. One possible explanation is that the strong model may already possess sufficient capacity to capture adversarial robustness independently, or the differences in model capacities may affect the dynamics of knowledge transfer.
On the other hand, increasing the weak model size from 14M to 70M generally led to improvements in the weak models trustworthiness during the Weak TFT and Weak+WTS TFT phases for both OOD robustness and adversarial robustness. This is expected, as larger weak models have greater capacity to learn complex patterns and trustworthiness properties, providing better supervision for the strong models.

\textbf{Sensitivity to Regularization Strength ($\lambda$).}
\ls{make less wordy, emphasis on robustness to lambda}
We also investigated how varying the regularization strength in the trustworthiness loss functions affects the transfer of trustworthiness properties. For each property—fairness, robustness, and privacy—we experimented with a range of $\lambda$ values to observe their impact on both the weak and strong models.
The weak-to-strong trustworthiness trends described in the previous section maintained across $\lambda$ values in the Weak+WTS TFT phase. The plots of trustworthiness metrics against varying lambda values showed consistent improvements in the WTS-Naive and WTS-Aux-Loss models' trustworthiness attributes when both weak and WTS models were regularized (Figure \ref{fig:lambda_phase3}). This consistency suggests that the effectiveness of the Weak+WTS TFT approach is robust to the choice of lambda, provided it is within a reasonable range.
Moving from the Weak TFT to the Weak+WTS TFT phase generally made the weak-to-strong trends more apparent across different lambda values. This behavior confirms our analysis in Section 4.1 that weak-to-strong trends are enhanced with increased regularization. Applying trustworthiness regularization to both the weak and strong models amplified the transfer of trustworthiness properties from Figure \ref{fig:lambda_phase2} to Figure \ref{fig:lambda_phase3}.

% Overall, our sensitivity analysis underscores several key insights:

% 1. Robustness of Weak-to-Strong Trends: The weak-to-strong trends in transferring trustworthiness properties are generally robust across different model sizes, especially for fairness and OOD robustness.

% 2. Limitations with Larger Weak Models in Adversarial Robustness: The disruption of weak-to-strong trends in adversarial robustness when using larger weak models (70M) suggests that the effectiveness of trustworthiness transfer may vary depending on the relative capacities of the weak and strong models.

% 3. Importance of Regularization in Both Models: Applying trustworthiness regularization to both the weak and strong models enhances the transfer of trustworthiness properties, making the trends more apparent across various lambda values.

% 4. Careful Selection of Alpha: The auxiliary loss weighting parameter alpha significantly impacts the performance of the strong models. Lower alpha values facilitate better adherence to the weak model's trustworthiness attributes.

% These insights highlight the complexity of transferring trustworthiness properties and emphasize the need to tailor fine-tuning strategies to the specific models and properties of interest. By understanding these nuances, we can better design approaches that maximize the benefits of weak-to-strong trustworthiness transfer while mitigating potential drawbacks.

==> section1.tex <==
% \hl{\begin{enumerate}
%     \item Para 1: intro about proliferation of gen AI, LLMs, and the emergent behaviors of LLMs
%     \item Para 2: one such emergent behavior is weak to strong generalization. Give a concrete example of old weak to strong
%     \item Para 3: motivate trustworthiness as another key aspect esp as LLMs are used in critical applications.
%     \item So argue that exploring whether weak to strong phenomenon holds with trustworthiness properties is an important direction but unexplored..
%     \item Para 4: in this work we address the aforementioned question and explore...To this end, we leverage framework built by openai but also develop two novel strategies and describe them
%     \item Para 5: we conducted rigorous experimental evaluation with multiple real world datasets such as... our results demonstrate that...
% \end{enumerate}}

Over the past few years, there has been a rapid proliferation of generative artificial intelligence (AI), particularly large language models (LLMs) like GPT-3, GPT-4, and their successors. These models have demonstrated remarkable capabilities across a wide range of tasks, including language comprehension \citep{radford2019language}, reasoning \citep{bubeck2023sparks} and tabular data generation \citep{borisov2022language}. Their emergent behaviors -- unexpected capabilities that arise as models scale -- have captured the attention of both academia and industry, leading to widespread adoption and integration into various applications \citep{wei2022emergent,schaeffer2024emergent}.

One intriguing key phenomenon observed in LLMs is known as weak-to-strong generalization \citep{burns2023weak}. 
In this context, a ``weak" model, typically smaller or less capable, is used to supervise the training of a larger-sized ``weak-to-strong" model. Remarkably, this larger model often surpasses the weak model in performance, even when trained solely on the weak model's outputs. 
For example, prior research has shown that when a large model is fine-tuned on the predictions of a smaller teacher model for tasks like sentiment analysis or machine translation, the larger model not only learns the task but also generalizes better to new, unseen data \citep{burns2023weak}.

While performance improvements are valuable, trustworthiness has emerged as a critical aspect of AI systems, especially as LLMs are increasingly deployed in high-stakes domains like healthcare, finance, and legal services \citep{wang2023decodingtrust}.
Trustworthiness encompasses properties such as fairness (avoiding biases against certain groups), privacy (protecting sensitive information), and robustness (maintaining performance under adversarial conditions or distribution shifts). Ensuring these properties is essential to prevent harmful outcomes, comply with regulations, and maintain public confidence in AI technologies.
Given the importance of trustworthiness, a vital yet unexplored question arises.
% centers the figure
\sidecaptionvpos{figure}{c}
\begin{SCfigure}
\centering
\includegraphics[width=.50\linewidth]{figures/teaser_wts.pdf}
\caption{\textbf{Weak-to-strong transfer strategies}.
We explore the transfer of trustworthiness properties to strong models using different weak-to-strong transfer approaches. 
\textbf{Top}: In \emph{No TFT}, both the weak and WTS models are finetuned solely for task performance.
\textbf{Middle}: In \emph{Weak TFT}, the weak model is fine-tuned for both task performance and trustworthiness, while the WTS model is finetuned only for task performance.
\textbf{Bottom}: In \emph{Weak+WTS TFT}, both models are fine-tuned for task performance and trustworthiness.}
\label{fig:teaser}
\end{SCfigure}


% Given the importance of trustworthiness, a vital yet unexplored question arises: Does the weak-to-strong generalization phenomenon extend to trustworthiness properties? Specifically, can a strong model inherit and potentially enhance fairness, privacy, and robustness from a weak model through fine-tuning on the weak model's outputs? Addressing this question is crucial for developing AI systems that are not only performant but also ethically aligned and reliable in critical applications.

\newtcolorbox{question}[2][]{center,%
    colframe=green!0!black,
    colback=green!0,
    enhanced,
    attach boxed title to top left={xshift=0.5cm, yshift=-3mm},
    colbacktitle=green!0,
    coltitle=green!0!black,
    title=#2}
\begin{question}{}
\centering 
% Does the weak-to-strong generalization phenomenon extend to trustworthiness properties? \\
\emph{\textbf{Research Question}: Can a strong model inherit or potentially enhance fairness, privacy, and robustness from a weak model through fine-tuning on trustworthy weak model outputs?}
\end{question}

% In this work, we investigate this critical question by exploring the transfer of trustworthiness properties from weak to strong models. More specifically, we examine whether a strong model can not only learn task performance from a weak model but also inherit and improve upon its trustworthiness attributes (see Figure \ref{fig:teaser}). To this end, we leverage the weak-to-strong generalization framework and introduce two novel fine-tuning strategies aimed at enhancing trustworthiness transfer:
% \begin{enumerate}[leftmargin=5mm]
% \item \textbf{Weak Trustworthiness Finetuning (Weak TFT)}: We apply trustworthiness regularization during the fine-tuning of the weak model. This involves modifying the loss function to include fairness constraints or robustness penalties.
% \item \textbf{Weak and Weak-to-Strong Trustworthiness Finetuning (Weak+WTS TFT)}: In addition to a regularized weak model, we add trustworthy weak-to-strong transfer to finetune the strong model using a trustworthiness regularizer on the weak labels.
% \end{enumerate}
% We conducted rigorous experimental evaluations using multiple real-world datasets: Adult (fairness), OOD Style Transfer (OOD robustness), AdvGLUE++ (adversarial robustness), Enron Emails (privacy).
% Our results demonstrate that while naive fine-tuning of the strong model on the weak model's outputs leads to only partial transfer of trustworthiness properties, the application of our proposed strategies significantly enhances this transfer. Specifically, strong models not only retain but also amplify fairness and robustness attributes when both models are regularized. In fairness experiments, the strong model achieved a lower demographic parity difference compared to the weak model, indicating improved fairness. Similarly, robustness assessments showed that the strong model was more resilient to adversarial perturbations and out-of-distribution shifts. 

\change{In this work, we investigate this critical question by exploring the generalization of trustworthiness properties from weak to strong models, a process we term \emph{weak-to-strong trustworthiness generalization}. 
We specifically examine whether a strong model can inherit and enhance the trustworthiness properties of a weak model, in addition to improving task performance.
To this end, we introduce two novel fine-tuning strategies aimed at enhancing trustworthiness transfer.
First, we apply trustworthiness regularization during the fine-tuning of the weak model only. 
This involves modifying the loss function of the weak model to include fairness, robustness or privacy constraints.
We refer to this training strategy as \emph{Weak Trustworthiness Fine-tuning} (Weak TFT).
Second, in addition to using a trustworthiness regularized weak model, we also add trustworthiness regularization to the weak-to-strong transfer where we finetune the weak-to-strong model using a trustworthiness regularizer on the trustworthy weak labels.
We call this second strategy \emph{Weak and Weak-to-Strong Trustworthiness Fine-tuning} (Weak+WTS TFT). 
These training strategies are summarized in Figure \ref{fig:teaser}.}

\change{We conduct rigorous empirical experiments using the Pythia model suite \citep{biderman2023pythia} to evaluate these training strategies on multiple real-world datasets including Adult (fairness), OOD Style Transfer (OOD robustness), AdvGLUE++ (adversarial robustness), and Enron Emails (privacy).
Our results demonstrate that while naive fine-tuning of the strong model on the standard weak model outputs only leads to limited weak-to-strong trustworthiness, our proposed training strategies significantly enhance weak-to-strong trustworthiness.
Specifically, strong models not only retain but also consistently amplify fairness and robustness properties when both models are regularized. 
In summary, our contributions can be summarized as follows:}
\change{
\begin{itemize}[leftmargin=10mm]
% \item \textbf{Weak Trustworthiness fine-tuning (Weak TFT)}: We apply trustworthiness regularization during the fine-tuning of the weak model. This involves modifying the loss function to include fairness constraints or robustness penalties.
% \item \textbf{Weak and Weak-to-Strong Trustworthiness fine-tuning (Weak+WTS TFT)}: In addition to a regularized weak model, we add trustworthy weak-to-strong transfer to finetune the strong model using a trustworthiness regularizer on the weak labels.
\item \textbf{Novel Trustworthy Learning Paradigm:} 
This is the first work to investigate if trustworthiness properties can transfer from a weak to a strong model using weak-to-strong supervision, a process we term \emph{weak-to-strong trustworthiness generalization}.
\item \textbf{Foundational Training Strategies for Weak-to-Strong Trustworthiness Generalization}: We introduce two baseline training strategies, Weak TFT and Weak+WTS TFT, designed to facilitate weak-to-strong trustworthiness generalization.
\item \textbf{Weak-to-Strong Trustworthiness Generalization is Feasible}: Our experiments show that some trustworthiness properties can indeed be generalized and even enhanced from weak to strong models.
\end{itemize}
}
Our findings provide new insights into systematically transferring and scaling trustworthiness properties from weaker to stronger models. They suggest a viable pathway for developing trustworthy AI systems without requiring full access to model internals or extensive human supervision. By demonstrating that trustworthiness can be effectively inherited and even enhanced through weak-to-strong generalization, we contribute to the foundational understanding necessary for aligning powerful AI systems with ethical principles.

==> section3.tex <==
We now present our methodology for investigating the generalization of trustworthiness properties from weak to strong models.
Our approach systematically explores whether and how fairness, privacy, and robustness can be effectively generalized from weaker to stronger models. 
The broader issue we address is: Under what conditions can a weaker model, despite its limitations, most effectively transfer properties such as fairness, privacy, and robustness to a more powerful model?
We begin by outlining the weak-to-strong training process, followed by techniques for eliciting specific trustworthiness properties in language models. 
Finally, we introduce a simple yet effective three-stage training approach that allows us to examine weak-to-strong trustworthiness generalization under different fine-tuning strategies.

% A key challenge in superalignment is the need for humans to supervise models that are far more intelligent than we are \citep{burns2023weak}. 
% In the context of trustworthy AI, this raises the question of how to guide these highly capable models toward ethical and robust behavior when the supervision comes from weaker, less capable models.
% In this work, we explore this question by conducting a series of experiments where a weak model, using only its outputs, acts as a mentor for a stronger model. 
% The goal is to examine whether trustworthiness properties can be transferred from a weak model to a strong one, and under what conditions such transfer is most effective.

\subsection{Preliminaries}

Here we present the key training strategies that underlie our work. 
First, we discuss how we adapt the weak-to-strong generalization framework introduced by \citet{burns2023weak}.
Following this, we examine widely-used regularization strategies for machine learning models aimed at enhancing trustworthiness properties such as robustness, fairness, and privacy.

\change{
\textbf{Notation.} We consider training datasets of the form $\{(x_i,y_i)\}_{i=1}^N$ where $y_i \in \mathcal{Y}$ is the ground-truth label and $a_i \in \{0,1\}$ represents a protected attribute (e.g., race or gender) that may be included in the features $x_i$.
We denote a classifier $f_\theta : \mathcal{X} \to \mathcal{Y}$ parametrized by $\theta \in \mathbb{R}^d$, mapping inputs $x \in \mathcal{X}$, to labels $\mathcal{Y}$. 
We define the outputs of a smaller, already trained, fixed classifier 
$f_w(x)$ as \emph{weak labels}, where $w \in \mathbb{R}^k$ denotes a lower-capacity parameterization than $\theta$ where $k \ll d$.   
Additionally, let $\ell: \mathbb{R} \times \mathbb{R} \to \mathbb{R}$ represent an appropriate loss function such as cross-entropy loss.
}

\textbf{Weak-to-Strong Training.}
In this framework, knowledge transfer from a large pre-trained model occurs by fine-tuning it on the labels produced by a smaller model. This process incorporates an additional auxiliary confidence loss, weighted by $\alpha \in [0,1]$ that adjusts the confidence in the strong model's predictions relative to the weak labels. 
This auxiliary loss encourages the strong model to make confident predictions, even when they diverge from the weak labels, potentially enhancing generalization.
The loss function is defined as a linear combination of the cross-entropy losses from the weak and strong models:
The loss function adapted to our weak-to-strong trustworthiness setting is defined as a linear combination of the losses from the trustworthy weak and strong models
\change{\begin{equation}
\ell_{\text{WTS-AUX}}(x, f_\theta; \alpha, \lambda, f_w) = (1 - \alpha) \cdot \ell\big(f_\theta(x), f_w(x;  \lambda)\big) + \alpha \cdot \ell\big(f_\theta(x; \lambda), \hat{f}_{t, \theta}(x)\big),
\label{eq:objective_trustworthy_wts}
\end{equation}
where $f_w(x; \lambda)$ is the fixed trustworthy weak model previously trained with trustworthiness property regularization strength $\lambda$ and $f_\theta(x)$ denotes the strong model.
Further, $\hat{f}_{t, \theta}(x)$ represents the hardened strong model predictions according to threshold $t$ that is set proportional to the class weights for each dataset. 
When $\lambda=0$, we are in the standard weak-to-strong setting previously studied by \citet{burns2023weak}.
When $\alpha=0$, we refer to the loss as $\ell_{\text{Naive}}$ since we train on the outputs of the weak model only.
In the following, we describe how we obtain the weak trustworthy models $f_w(\cdot; \lambda)$ through various regularization techniques aimed at improving trustworthiness.
}

\textbf{Fairness.} Here we discuss how we can enhance fairness through regularization using a widely-used fairness notion known as Demographic Parity which requires:
\begin{align}
\mathbb{P}(f_w(x) = 1 | a = 1) = \mathbb{P}(f_w(x) = 1 | a = 0).
\label{eq:demographic_parity}
\end{align}
To enforce this fairness constraint during finetuning, we use the following objective function from \citet{zafar2017fairness},
\begin{align}
\min_w \mathcal{L}_{\text{Fair}}(w; \lambda_{\text{Fair}}) = \min_w \frac{1}{N} \sum_{i=1}^N \ell(f_w(x_i), y_i) + \lambda_{\text{Fair}} \cdot  (a_i - \bar{a}) \cdot f_w(x_i),
\label{eq:fairness_regularizer}
\end{align}
where $\bar{a} = \frac{1}{N} \sum_{i=1}^N a_i$ is the base rate of the protected attribute. 
The first term in \eqref{eq:fairness_regularizer} encourages to make correct predictions while the second term acts as a fairness regularizer.
Specifically, this term minimizes the covariance between the protected attribute $a_i$ and the model outputs $f_w(x_i)$, encouraging the model to satisfy demographic parity by becoming independent of the protected attribute $a$.
The hyperparameter $\lambda_{\text{Fair}}$ controls the tradeoff between prediction accuracy and fairness where a higher value of $\lambda_{\text{Fair}}$ encourages more emphasis on achieving fairer outcomes. 

\textbf{Adversarial Robustness.}
% \ak{Machine learning models, such as deep neural networks, are known to malfunction under small, adversarial changes in their inputs \citep{Szegedy2014, GoodfellowSS14, MadryMSTV18}.
% Such adversarial inputs are generated using optimization procedures that seek to change the output of a model by introducing minimal perturbations to a benign input.
% Large language models (LLMs), being deep neural networks, are not exempt from this vulnerability. Several adversarial attack algorithms have been developed that can degrade an LLM's performance on natural language processing tasks such as sentiment analysis, question answering, text classification, and entailment \citep{JinJZS20, ZangQYLZLS20, wang2020t3, li2020bertattack, garg2020bae}.
% }
In adversarial training, adversarially perturbed samples are introduced during the training process, enabling the model to learn to become invariant to small input perturbations and thereby become more robust to adversarial attacks.
In this setting, the training dataset consists of triplets $(x, x', y)$, where $x$ is a clean input sample, $x'$ is an adversarially manipulated version of $x$ and $y$ is the ground truth label of $x$.
%We denote the $i^{th}$ training sample as $(x_i, x'_i, y_i)$.
% As before, let $f_w$ represent the model and $\ell$ be a loss function (e.g., cross-entropy loss) that measures the model's prediction accuracy. 
The training objective combines the losses from both clean and adversarial samples:
\begin{align}
\min_w \mathcal{L}_{\text{Adv}}(w; \lambda_{\text{Adv}}) = \min_w \; \frac{1}{N} \sum_{i=1}^N(1-\lambda_{\text{Adv}}) \cdot \ell(f_{w}(x_i), y_i) + \lambda_{\text{Adv}} \cdot \ell(f_w(x'_i), y_i),
\end{align}
 where $\lambda_{\text{Adv}}$ controls the tradeoff between clean and adversarial losses. 
A higher $\lambda_{\text{Adv}}$ places greater emphasis on robustness to adversarial perturbations.


\textbf{Out-of-distribution robustness.} 
We use embedding perturbations as the method to enhance out-of-distribution robustness, following approaches from \citet{advembed, lecuyer2019certified, zhu2019freelb}.
Specifically, we experiment with a setting that adds i.i.d.\ Gaussian noise to the word embeddings \citep{bowman2015generating, li2019certified}.
Define \(e(x) \in \mathbb{R}^{d} \) as the word embedding of input \( x \), where \( d \) is the embedding dimension.
We add Gaussian noise \(z \sim \mathcal{N}(0, \lambda_{\text{OOD}} \cdot \text{I}_d) \) drawn from a distribution with mean $0$ and covariance matrix \( \lambda_{\text{OOD}} \cdot \text{I}_d\) to the word embedding which yields a noisy embedding: \(\tilde{e}(x; \lambda_{\text{OOD}}) = e(x) + z \).
This noisy embedding is then used to finetune the model.
Here, let \( f_w(x; \lambda_{\text{OOD}}) = g_{w}(\tilde{e}(x; \lambda_{\text{OOD}})) \) be the output of the language model parametrized by $w$. 
The objective during finetuning is to minimize the following loss:
\begin{align} 
\min_w \mathcal{L}_{\text{OOD}}(w; \lambda_{\text{OOD}}) = \min_{w} \frac{1}{N} \sum_{i=1}^N \ell\big(y_i, f_w(x_i; \lambda_{\text{OOD}}))\big),
\end{align}
where $\lambda_{\text{OOD}}$ controls the strength of the OOD regularizer. 
As $\lambda_{\text{OOD}} \to 0$ the model is trained without any regularization, reverting to the vanilla model. 

\textbf{Privacy.}
In $(\lambda_P,\delta)$-differential privacy, the goal is to ensure that the output of an algorithm $\mathcal{A}$ is nearly indistinguishable whether or not any single data point is included in the dataset. 
Specifically, for any two datasets $D_1$ and $D_2$ that differ by only one element, the algorithm $\mathcal{A}$ satisfies $(\lambda_P,\delta)$-differential privacy if:
\begin{align}
\mathbb{P}(\mathcal{A}(D_1) \in S) \leq \exp(\lambda_P) \cdot \mathbb{P}(\mathcal{A}(D_2) \in S) + \delta,
\end{align}
for any possible output set $S$. 
Here, $\lambda_P$ controls the privacy loss, with smaller values indicating stronger privacy guarantees, while $\delta$ allows for a small probability of the privacy guarantee being violated.
To operationalize $(\lambda_{P}, \delta)$-differential privacy, we use the most popular privacy algorithm called DP-SGD as in the work by \citet{abadi2016deep}.
DP-SGD is a variant of classical SGD that comes with privacy guarantees.
In summary, the algorithm consists of three fundamental steps: 
\emph{gradient clipping} with clipping constant $C$, i.e., $\gamma = g(x_i, y_i) \cdot\max(1, C/\lVert g(x_i, y_i)\rVert)$ where $g(x_i, y_i) = \nabla_w \mathcal{L}(x_i, y_i)$ is the gradient of the loss function $\ell$ with respect to the model parameters,
\emph{aggregation} (i.e., $m = \frac{1}{n}\sum_{i=1}^n \gamma_i$) and
\emph{adding Gaussian noise} (i.e., $\tilde{m} = m + Y$ where $Y \sim \mathcal{N}(0, \tau^2 \text{I})$ with variance parameter $\tau^2$).
By carefully tuning the noise level $\tau^2$, we ensure that the model satisfies the privacy guarantees specified by the parameters $\lambda_{P}$ and $\delta$.

\subsection{Eliciting Weak-to-Strong Trustworthiness in Large Language Models}
\label{sec:wts_trustworthy_training}

We break the analysis into three stages, each building on the last by varying the regularization applied to the weak and weak-to-strong models.

% \ak{Suggestion for phase names:
% \begin{itemize}
%     \item Phase 1: No Trustworthiness Fine-Tuning (No TFT)
%     \item Phase 2: Weak (model) TFT
%     \item Phase 3: Weak + Weak-to-Strong TFT (Weak + WTS TFT)
% \end{itemize}
% }

\textbf{No trustworthiness finetuning (No TFT).}
In this phase, we establish baseline performance by training the weak, strong, and weak-to-strong models without applying any trustworthiness regularization, following the approach outlined in \citet{burns2023weak}:
\begin{enumerate}[label=\(\bullet\), leftmargin=4mm, nosep]
\itemsep0.10cm
\item \textbf{Weak model:} 
We use small, pretrained LLMs as weak supervisors, referred to as weak models.
These weak models are finetuned on ground truth labels to generate predictions. 
Using the finetuned weak models, we create weak labels by having the weak models make predictions on a held-out validation set.
\item \textbf{Weak-to-strong transfer:}  
To evaluate weak-to-strong generalization, we fine-tune a strong model using the weak labels generated by the weak model. 
This model is referred to as the strong student, and its resulting performance is called the weak-to-strong performance.
% \item \textbf{Strong ceiling:} 
% For comparison, we also fine-tune a strong model using the actual ground truth labels. 
% This is referred to as the strong ceiling model, and its performance represents the upper bound of what the strong model can achieve when fully utilizing its capabilities on the task.
\end{enumerate}

\textbf{Weak trustworthiness finetuning (Weak TFT).}
In this phase, we explore whether a trustworthiness regularized weak model can influence the trustworthiness property of a vanilla strong model trained solely on the output of the trustworthy weak model:
\begin{enumerate}[label=\(\bullet\), leftmargin=4mm, nosep]
\itemsep0.10cm
\item \textbf{Trustworthy weak model:}
We use small, pre-trained LLMs as weak supervisors, but unlike in Phase 1, these weak models are fine-tuned on ground truth labels using a trustworthiness regularizer. 
This regularizer enforces specific trustworthiness properties, such as fairness, privacy, or robustness, during fine-tuning. These models are referred to as trustworthy weak models.
Using these models, we generate weak labels by making predictions on a held-out validation set.
\item \textbf{Weak-to-strong transfer:} 
To assess whether trustworthiness properties can be transferred from a weak to a strong model, we fine-tune a vanilla strong model using the weak labels generated by the trustworthy weak model. 
% This model is called the implicit trustworthy strong student, and its performance, referred to as implicit trustworthy weak-to-strong performance, reflects how well the strong model incorporates trustworthiness properties from the weak model.

% \item \textbf{Trustworthy strong ceiling:} 
% For comparison, we fine-tune a trustworthy strong model using the ground truth labels, applying the same trustworthiness regularizer used for the weak model. 
% This model is called the trustworthy strong ceiling model, and its performance represents the maximum possible capability of the strong model when trained with both ground truth labels and trustworthiness properties.
\end{enumerate}

\textbf{Weak and weak-to-strong trustworthiness finetuning (Weak+WTS TFT).}
In the final phase, we investigate whether adding trustworthiness regularization to both the weak and weak-to-strong models can further enhance trust transfer (and performance).
\begin{enumerate}[label=\(\bullet\), leftmargin=4mm, nosep]
\itemsep0.10cm
\item \textbf{Trustworthy weak model:} The trustworthy weak model is the same as in Phase 2, where the weak model is fine-tuned on ground truth labels using a trustworthiness regularizer to enforce properties like fairness, privacy, or robustness.
\item \textbf{Trustworthy weak-to-strong transfer:}
In this step, we directly assess how well trustworthiness properties can be transferred from the weak model to the strong model. Unlike in Phase 2, where the strong model was fine-tuned without any regularization, here we finetune the strong model using a trustworthiness regularizer on the weak labels generated by the trustworthy weak model. 
 % This model is referred to as the doubly trustworthy strong student, and its performance, called doubly trustworthy weak-to-strong performance, measures how effectively the strong model incorporates trustworthiness properties when both models are regularized.
% \item \textbf{Trustworthy strong ceiling:} The trustworthy strong ceiling model is the same as in Phase 2, where the strong model is fine-tuned on ground truth labels with trustworthiness regularization, representing the upper limit of performance with respect to trustworthiness.
\end{enumerate}




% \begin{figure}
% \centering

% \input{figures/tikz/fig1}

% \caption{\textbf{Model training overview}. The weak model $f_w$ is trained on $D_{\text{W}}=\{(x_i,y_i)\}$. Subsequently, we use the weak model $f_w$ to label the second, unlabeled training dataset $D_{\text{WTS}} =\{(x_i, y_i)\}$ resulting in $D_{\text{WTS}'} = \{(x_i, f_w(x_i))\}$. We use $D_{\text{WTS}'}$ to train the weak-to-strong model $f_\theta$.}
% \label{fig:training_data_flow}

% \end{figure}


% \begin{figure}
% \centering

% \input{figures/tikz/fig2}

% \caption{\textbf{Model evaluation overview}.}
% \label{fig:evaluation_data_flow_all_but_privacy}

% \end{figure}

==> section4.tex <==
In Section \ref{sec:experiments_main}, we empirically evaluate the effectiveness of generalizing trustworthiness properties from a weak to a strong model using the three weak-to-strong training strategies introduced in the previous section.
Then, in Section \ref{sec:experiments_sensitivity}, we perform a thorough sensitivity analysis, varying the trustworthiness regularization strength, model size, and key hyperparameters specific to weak-to-strong transfer training. 
We begin by describing the real-world datasets used in our experiments, followed by an overview of the LLMs and relevant baselines used for comparison.

\textbf{Datasets.} 
We evaluate the transfer of trustworthiness properties from small models to large models using four datasets, previously explored by \citet{wang2023decodingtrust}, including the Enron Email dataset \citep{klimt2004enron}, the Adult dataset \citep{ding2021retiring}, the OOD Style Transfer dataset \citep{wang2023decodingtrust}, and the AdvGLUE++ dataset \citep{wang2023decodingtrust}. 
For all datasets, we show average results over multiple runs and usually report $\pm 1$ standard deviation across runs. 
\begin{enumerate}[label=\(\bullet\), leftmargin=3mm, nosep]
\itemsep0.10cm
\item \textbf{Enron Emails}: This dataset contains over 600,000 emails generated by employees of the Enron Corporation.
This dataset includes sensitive personal information, such as email addresses, phone numbers, credit card numbers, and Social Security Numbers, which could be memorized and extracted by language models. 
For finetuning, we randomly subsampled 10,000 data points.
\item \textbf{Adult}: This dataset is derived from the 1994 U.S. Census database and contains 48,842 instances with 14 attributes.
The task is to classify whether an individual’s income exceeds \$50,000 (USD) per year. We use the reconstructed Adult dataset provided by \citet{ding2021retiring} and selected the ``sex'' feature as the protected attribute to evaluate fairness-related properties.
\item \textbf{OOD Style Transfer}: This dataset is based on the SST-2 sentiment classification dataset but incorporates a variety of text and style transformations. 
The transformations (e.g., shifts in language style, vocabulary, syntax, and tone) are applied at both the word and sentence level while preserving the original meaning. 
For instance, some transformations involve substituting words with Shakespearean equivalents.
The task is to correctly classify the sentiment of inputs. %despite these style transformations.
\item \textbf{AdvGLUE++}: This dataset contains clean and adversarial input 
samples for six NLP tasks: Sentiment analysis (SST-2), duplicate question detection (QQP), multi-genre natural language inference (MNLI, MNLI-mm), recognizing textual entailment (RTE), and question answering (QNLI).
It contains around 2K to 15K samples for each of the six tasks.
We randomly sample up to 10K samples for each task and aggregate the performance of the model by averaging over these six tasks.
\end{enumerate}

\textbf{Large Language Models.} We conduct our experiments using the Pythia model suite \citep{biderman2023pythia}, which includes models of varying scales (14M, 70M, 410M, 1B). 
This allows us to systematically explore how model size impacts the effectiveness of trustworthy weak-to-strong generalization. 
For each model, we finetune on classification tasks by adding a classification head on top of the second-to-last layer. 
The models are trained using the standard cross-entropy loss. %, with an initial learning rate of $5 \cdot 10^{-5}$.

\textbf{Metrics} 
% \ls{define f, theta?}
For \emph{fairness}, we evaluate the finetuned LLMs  using the Demographic Parity Difference (DPD) defined as
$\text{DPD} = \mathbb{P}(f_\theta(x) = 1 | a = 1) = \mathbb{P}(f_\theta(x) = 1 | a = 0)$.
A smaller DPD indicates better fairness, as it reflects minimal disparity in predictions between the two protected groups.
For \emph{robustness}, we measure both OOD accuracy and adversarial accuracy, abbreviated as Robust Accuracy (RA), by evaluating the model's performance on OOD and adversarially perturbed test data.
Specifically, we compute the $\text{RA} = \frac{1}{n_{\text{test}}} \sum_{i=1}^{n_{\text{test}}} \mathbb{I}[f_\theta(x_i') = y_i]$, where $x'$ represents either an OOD sample or an adversarially perturbed input, and  $\mathbb{I}$ is the indicator function that equals 1 if the prediction is correct.
For \emph{privacy}, we evaluate the models using targeted data extraction attacks \citep{carlini2021extracting}.
In this attack, given a prefix sequence and a generated response of $k$ tokens, we compute the extraction rate by determining how many of the $k$-token continuation (suffix) matches the ground truth continuation of the sample. 
A higher extraction rate indicates a greater risk of private information being memorized and extracted by the model.

\textbf{Baselines.}
For comparison, we establish reference points for both trustworthiness and task performance.
To provide a benchmark, we fine-tune a strong model using ground truth labels with varying levels of trustworthiness regularization. 
We then select the model that achieves the best trade-off between task performance and trustworthiness. 
We provide an illustrative example of this selection procedure in Figure \ref{fig:tradeoff}.
This model, referred to as the \emph{strong ceiling}, represents the empirical upper bound of the strong model’s capabilities for both task performance and trustworthiness.

\begin{figure}[tb]
\centering
\begin{subfigure}{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/fairness_main_results.png}
\caption{Fairness}
\label{fig:main_fairness}
\end{subfigure}~
\begin{subfigure}{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/ood-main.pdf}
\caption{OOD Robustness}
\label{fig:main_ood_rob}
\end{subfigure}~
\begin{subfigure}{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/pythia-14m-410m-ep6.png}
\caption{Adv.\ Robustness}
\label{fig:main_adv_rob}
\end{subfigure}~
\begin{subfigure}{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/privacy_main_plot_14-410.png}
\caption{Privacy}
\label{fig:main_privacy}
\end{subfigure}

\caption{\textbf{Weak-to-strong trustworthiness for Pythia 14M/410M models}. {Trustworthiness properties and task performance for our four properties: Fairness, OOD Robustness, Adversarial Robustness, and Privacy. Note that lower values are better for the top plot in Figure \ref{fig:main_fairness} as the y-axis is Unfairness (DPD). Similarly, lower values are better for the top plot in Figure \ref{fig:main_privacy} as the the y-axis is Extraction Rate.} Results for WTS-Aux-Loss for privacy are omitted since it was the only task involving free data generation, making the auxiliary loss function inapplicable.}
\label{fig:experiment_main}
\end{figure}

\subsection{Evaluating Trustworthiness of the Weak to Strong Model}
\label{sec:experiments_main}


\begin{figure}[tb]
\centering
\begin{subfigure}{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/fairness_lambda_phase3.png}
\caption{Fairness}
\label{fig:fairness_lambda_phase3}
\end{subfigure}~
\begin{subfigure}{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/ood-lambda-phase3.pdf}
\caption{OOD Robustness}
\label{fig:ood_lambda_phase3}
\end{subfigure}~
\begin{subfigure}{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/phase3_sensitivity_plots.png}
\caption{Adv.\ Robustness}
\label{fig:adv_rob_lambda_phase3}
\end{subfigure}~
\begin{subfigure}{0.24\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/privacy_sensitivity_phase3.png}
\caption{Privacy}
\label{fig:privacy_lambda_phase3}
\end{subfigure}
\caption{\textbf{Varying Lambda for Weak+WTS TFT}. Results for WTS-Aux-Loss for  privacy are omitted since it was the only task involving free data generation, making the auxiliary loss function inapplicable.}
\label{fig:lambda_phase3}
\end{figure}


%\map{First pass complete. Potentially talk about task performance.}
We present our results for all four trustworthiness properties across the three phases in Figure \ref{fig:experiment_main}. For each property, we used Pythia 14M as the weak model and Pythia 410M as the strong model.

\textbf{No TFT.}
% \ls{takeaway first sentence? or italics?}
In the initial No TFT phase, where models are trained without any trustworthiness regularization, we expected no clear trustworthy weak-to-strong transfer trends, as no regularization is in place to explicitly enforce trustworthiness properties.
Surprisingly, for both OOD and adversarial robustness evaluation we observe that the models demonstrate a trustworthy weak-to-strong trend. 
Despite the absence of regularization, the stronger models exhibited improved robustness compared to the weaker models, suggesting that some trustworthiness properties may naturally transfer even without explicit constraints.
For fairness, we do not observe a trustworthy weak-to-strong trend. 
The level of unfairness remains constant, regardless of whether we examine the weak model or the weak-to-strong transfer model.  


% \begin{important}
% \centering 
% Without trustworthy fine-tuning we observe inconsistent weak-to-strong trustworthiness trends.
% \end{important}

%On the task performance side, only the models for OOD robustness and privacy displayed weak-to-strong trends. Their WTS-Naive model outperforms their weak model in percentage of accurate predictions, with OOD robustness' WTS-Aux-Loss models achieving similar performance as the WTS-Naive models. There is no task performance weak-to-strong for fairness or adversarial robustness as their weak models slightly outperforms their WTS-Naive and WTS-Aux-Loss models. \ls{mention there is little gap between weak and strong performance in Phase 1?} 

\textbf{Weak TFT.}
In the Weak TFT phase, regularization is applied to the weak models, which, as expected, improves their trustworthiness in terms of fairness, OOD robustness, and adversarial robustness compared to the No TFT phase. 
This improvement aligns with our expectations, as the weak models are now being explicitly regularized to enhance their trustworthiness.
\emph{The only trustworthiness weak-to-strong trend observed in the Weak TFT phase pertains to OOD robustness.} 
In this case, the improvement is substantial, increasing robust accuracy from 72\% to 75\%, representing a gain of 3 percentage points.
For all other cases, we do not observe weak-to-strong trends.
For privacy, while we do not observe a trustworthy weak-to-strong trend, the gap in extraction rates between the WTS-Naive model and the weak model widens. 
This widening occurs because the smaller model benefits from privacy regularization, which limits the leakage of information about the training data. 
In contrast, the WTS-Naive model is trained without any regularization on a second, disjoint dataset, meaning the privacy guarantees from the first model's training phase do not apply. 
As a result, without explicit regularization during WTS training, the extraction rate for the explicitly regularized weak model decreases much more rapidly, dropping from 18\% to 14\%. In contrast, the implicitly regularized WTS-Naive model, trained on the outputs of the weak model, experiences a much smaller decline in extraction rate, from 45\% to 44\%.

%Weak TFT does not result in change in extraction rate or task performance for privacy. 

%we notice that the weak model trustworthiness improves relative to the No TFT phase. However, the only trustworthiness weak-to-strong trend in the Weak TFT phase is for OOD robustness.

\textbf{Weak+WTS TFT.} 
The Weak+WTS TFT phase introduces an additional layer of trustworthiness to the weak-to-strong transfer process, as the training of the WTS model itself is now regularized on top of the existing regularization applied to the weak model in the Weak TFT phase.
\emph{With both weak and weak-to-strong models fine-tuned using a trustworthiness regularizer, we observe consistent weak-to-strong trends for all trustworthiness properties, except for privacy.}
For fairness, OOD robustness, and adversarial robustness, we observe a statistically significant improvement of each property from weak models to WTS-Naive models. In addition, for fairness and adversarial robustness, there is an enhanced transfer from weak to WTS-Aux-Loss (where WTS-Aux-Loss is more trustworthy than WTS-Naive). 
For privacy, the extraction rate of the WTS-Naive model decreases by approximately 20 percentage points, dropping from 45\% to 26\%. 
This indicates an improvement in privacy compared to the WTS-Naive models from the No TFT and Weak TFT phases, attributed to the explicit regularization applied during WTS-Naive training.
However, despite this regularization, the WTS-Naive model remains less private than the weak model, which has an extraction rate of 14\%.


\change{\textbf{Remarks on the WTS Privacy Trends.} 
Privacy presents a unique situation. 
Note that the strong ceiling does not achieve better privacy than the weak model.
One reason for this is that privacy is measured with respect to the underlying training dataset (see Appendix \ref{app:dataset_and_eval_details} for a more detailed discussion on how the privacy evaluation differs from the evaluations of all other trustworthiness properties). 
Larger models, all else being equal, tend to memorize more information, leading to a greater risk of private information leakage \citep{leemann2024gaussian} and as a result larger models are more susceptible to leak private data than small models.
Therefore we observe that privacy, as measured by the extraction rate (or membership inference attack success in Figure \ref{fig:privacy_mia}), degrades when transferring knowledge from the smaller model to the larger model, primarily because privacy violations for the WTS model are measured for the larger model, which is more capable of memorizing its training data, rather than the smaller one.}


\textbf{Tradeoff Between Trustworthiness and Task Performance.} For fairness and adversarial robustness, improvements in trustworthiness come with a slight decline in task performance. However, the decrease in accuracy does not exceed 1.5\% across all phases for the two properties while the improvements in trustworthiness were up to 3 percentage points (equivalent to 60\% decrease in unfairness). This demonstrates that significant enhancements in trustworthiness can be achieved with minimal sacrifice to task performance.

% \citep{leemann2024gaussian}.
% The strong ceiling does not achieve better privacy than the weak model. While WTS-Naive model outperforms the weak model in task performance, we do not observe a weak-to-strong trend in privacy as the WTS-Naive model is less private than both the weak model and strong ceiling.
% \ls{@Martin, explain that Privacy has no WTS-Auxiliary, also elaborate on intuition for why WTS is not present even if you fine-tune for privacy, also touch upon how task performance is defined differently for weak and WTS models (trained dataset vs ground truth)}

% We observe a tradeoff between trustworthiness and task performance (accuracy on initial task) for all properties but OOD robustness. For fairness and adversarial robustness, trustworthiness for weak model improves from the No TFT phase to the Weak TFT and Weak+WTS TFT phases, resulting in a decline in weak model task performance. There is a similar tradeoff of a smaller scale for applying WTS-Naive and WTS-Auxiliary for fairness and adversarial robustness in Weak+WTS TFT phase: task performance declines by 1\% - 1.5\% but trustworthiness improves 2\% - 4\%. No tradeoff is present in OOD robustness as weak-to-strong methods significantly improve both robustness and task performance. 

\sidecaptionvpos{figure}{c}
\begin{SCtable}%[1]
%\begin{table}[tb]
\centering
\scalebox{0.90}{
\begin{tabular}{ccccc}
\toprule
& \textbf{Fairness}  & \textbf{\begin{tabular}[c]{@{}c@{}}OOD \\ Robustness\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Adv.\ \\ Robustness\end{tabular}} & \textbf{Privacy} \\ 
\midrule
\textbf{No TFT} & $\times$ & $\checkmark$ & $\checkmark$ & $\times $ \\ \midrule
\textbf{Weak TFT} & $\times$ &  $\checkmark$  & $\times$ & $\times$  \\ \midrule
\textbf{Weak+WTS TFT} &  $\checkmark$ &  $\checkmark$ &  $\checkmark$ & $\times$ \\ \bottomrule
\end{tabular}
}
\centering
\caption{\change{\textbf{Presence of weak-to-strong trustworthiness across trustworthiness properties for different training strategies described in Section \ref{sec:wts_trustworthy_training}.} 
% For the No TFT and Weak TFT training strategies, we observe inconsistent weak-to-strong trustworthiness. In Weak+WTS TFT stage, we observe consistent significant trustworthiness WTS across fairness, OOD robustness, and adversarial robustness. Privacy does not display trustworthiness WTS in any stage.
}}
\label{tbl:wts_table}
\end{SCtable}

\subsection{Sensitivity Analysis}
\label{sec:experiments_sensitivity}

In this section, we conduct a comprehensive sensitivity analysis to explore how various parameter values influence the transfer of trustworthiness properties from weak to strong models. Specifically, we examine the impact of different model sizes and the regularization strength ($\lambda_{\text{Fair}}, \lambda_{\text{Adv}}, \lambda_{\text{OOD}}, \lambda_P$) in the trustworthiness loss functions. We continue the sensitivity analysis for the auxiliary loss weighting parameter ($\alpha$) used during weak-to-strong transfer in Appendix \ref{sec:appendix_a}. This analysis aims to validate the robustness of our findings from the previous section and to understand the conditions under which weak-to-strong trustworthiness transfer is most effective.

\textbf{Sensitivity to Model Size.}
To assess the effect of model capacity on trustworthiness transfer, we experimented with different combinations of weak and strong model sizes. We analyzed experiments for four weak/strong configurations: Pythia 14M/410M, Pythia 14M/1B, Pythia 70M/410M, Pythia 70M/1B.
Our analysis reveals that the weak-to-strong trends observed in the previous section generally hold across these model sizes for most trustworthiness properties. Specifically, for fairness and OOD robustness, the strong models continued to inherit and, in some cases, enhance the trustworthiness attributes from the weak models across all configurations (Figure \ref{fig:fairness_model_size}, Figure \ref{fig:ood_robustness_model_size}).

%\ls{multiple claims made here, separate?}
However, we observed a disruption of the weak-to-strong trend for adversarial robustness when using 70M as the weak model. The weak-to-strong trend in adversarial robustness was disrupted in the Weak+WTS TFT phase in the 70M/410M and 70M/1B configurations; the strong models did not exhibit the expected improvement in adversarial robustness over the weak models (Figure \ref{fig:adversarial_robusness_model_size}). This contrasts with the results from using a 14M weak model, where the strong models did show enhanced adversarial robustness. This disruption suggests that as the weak model becomes more capable, the transfer of adversarial robustness to even stronger models may not follow the same patterns. One possible explanation is that the strong model may already possess sufficient capacity to capture adversarial robustness independently, or the differences in model capacities may affect the dynamics of knowledge transfer.
On the other hand, increasing the weak model size from 14M to 70M generally led to improvements in the weak models trustworthiness during the Weak TFT and Weak+WTS TFT phases for both OOD robustness and adversarial robustness. This is expected, as larger weak models have greater capacity to learn complex patterns and trustworthiness properties, providing better supervision for the strong models.



\textbf{Sensitivity to Regularization Strength ($\lambda$).}
% \ls{make less wordy, emphasis on robustness to lambda}
We also investigated how varying the regularization strength in the trustworthiness loss functions affects the transfer of trustworthiness properties. For each property—fairness, robustness, and privacy—we experimented with a range of $\lambda$ values to observe their impact on both the weak and strong models.
The trustworthiness weak-to-strong trends described in the previous section maintained across $\lambda$ values in the Weak+WTS TFT phase. The plots of trustworthiness metrics against varying lambda values showed consistent improvements in the WTS-Naive and WTS-Aux-Loss models' trustworthiness attributes when both weak and WTS models were regularized (Figure \ref{fig:lambda_phase3}). This consistency suggests that the effectiveness of the Weak+WTS TFT approach is robust to the choice of lambda, provided it is within a reasonable range.
Moving from the Weak TFT to the Weak+WTS TFT phase generally made the weak-to-strong trends more apparent across different lambda values. This behavior confirms our analysis in Section 4.1 that weak-to-strong trends are enhanced with increased regularization. Applying trustworthiness regularization to both the weak and strong models amplified the transfer of trustworthiness properties from Figure \ref{fig:lambda_phase2} to Figure \ref{fig:lambda_phase3}.

% Overall, our sensitivity analysis underscores several key insights:

% 1. Robustness of Weak-to-Strong Trends: The weak-to-strong trends in transferring trustworthiness properties are generally robust across different model sizes, especially for fairness and OOD robustness.

% 2. Limitations with Larger Weak Models in Adversarial Robustness: The disruption of weak-to-strong trends in adversarial robustness when using larger weak models (70M) suggests that the effectiveness of trustworthiness transfer may vary depending on the relative capacities of the weak and strong models.

% 3. Importance of Regularization in Both Models: Applying trustworthiness regularization to both the weak and strong models enhances the transfer of trustworthiness properties, making the trends more apparent across various lambda values.

% 4. Careful Selection of Alpha: The auxiliary loss weighting parameter alpha significantly impacts the performance of the strong models. Lower alpha values facilitate better adherence to the weak model's trustworthiness attributes.

% These insights highlight the complexity of transferring trustworthiness properties and emphasize the need to tailor fine-tuning strategies to the specific models and properties of interest. By understanding these nuances, we can better design approaches that maximize the benefits of weak-to-strong trustworthiness transfer while mitigating potential drawbacks.
